From Zero to Hero: Detecting Leaked Data through Synthetic Data Injection and Model Querying

Safeguarding the Intellectual Property (IP) of data has become critically important as machine learning applications continue to proliferate, and their success heavily relies on the quality of training data. While various mechanisms exist to secure data during storage, transmission, and consumption, fewer studies have been developed to detect whether they are already leaked for model training without authorization. This issue is particularly challenging due to the absence of information and control over the training process conducted by potential attackers. In this paper, we concentrate on the domain of tabular data and introduce a novel methodology, Local Distribution Shifting Synthesis (\textsc{LDSS}), to detect leaked data that are used to train classification models. The core concept behind \textsc{LDSS} involves injecting a small volume of synthetic data--characterized by local shifts in class distribution--into the owner's dataset. This enables the effective identification of models trained on leaked data through model querying alone, as the synthetic data injection results in a pronounced disparity in the predictions of models trained on leaked and modified datasets. \textsc{LDSS} is \emph{model-oblivious} and hence compatible with a diverse range of classification models. We have conducted extensive experiments on seven types of classification models across five real-world datasets. The comprehensive results affirm the reliability, robustness, fidelity, security, and efficiency of \textsc{LDSS}. Extending \textsc{LDSS} to regression tasks further highlights its versatility and efficacy compared with baseline methods.

==> tables/datasets.tex <==
\begin{table}[t]
\centering
\captionsetup{skip=0.5em}
\small
\caption{Statistics of the five datasets.}
\label{tab:data-stats}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccc} \toprule
  \textbf{Datasets} & \textbf{\# Samples} & \textbf{\# Cat. Feat.} & \textbf{\# Num. Feat.} & \textbf{\# Classes} & $g$ & $h$ \\ \midrule % & $d_c$ & $d_n$
  Adult     & 48,842    & 8   & 5   & 2  & 10  & 44    \\
  Vermont   & 129,816   & 40  & 8   & 4  & 10  & 118   \\
  Arizona   & 203,353   & 42  & 8   & 4  & 10  & 185   \\
  Covertype & 581,012   & 2   & 10  & 7  & 10  & 528   \\
  GeoNames  & 1,891,513 & 2   & 5   & 9  & 10  & 1,720 \\
  \bottomrule
\end{tabular}}
\end{table}

